Practical computation of the diffusion MRI signal of realistic neurons based on Laplace eigenfunctions

The complex transverse water proton magnetization subject to diffusion-encoding magnetic field gradient pulses in a heterogeneous medium such as brain tissue can be modeled by the Bloch-Torrey partial differential equation. The spatial integral of the solution of this equation in realistic geometry provides a gold-standard reference model for the diffusion MRI signal arising from different tissue micro-structures of interest. A closed form representation of this reference diffusion MRI signal has been derived twenty years ago, called Matrix Formalism that makes explicit the link between the Laplace eigenvalues and eigenfunctions of the biological cell and its diffusion MRI signal. In addition, once the Laplace eigendecomposition has been computed and saved, the diffusion MRI signal can be calculated for arbitrary diffusion-encoding sequences and b-values at negligible additional cost. Up to now, this representation, though mathematically elegant, has not been often used as a practical model of the diffusion MRI signal, due to the difficulties of calculating the Laplace eigendecomposition in complicated geometries. In this paper, we present a simulation framework that we have implemented inside the MATLAB-based diffusion MRI simulator SpinDoctor that efficiently computes the Matrix Formalism representation for realistic neurons using the finite elements method. We show the Matrix Formalism representation requires around a few hundred eigenmodes to match the reference signal computed by solving the Bloch-Torrey equation when the cell geometry comes from realistic neurons. As expected, the number of required eigenmodes to match the reference signal increases with smaller diffusion time and higher b-values. We gave the transformation that links the Laplace eigenfunctions to the eigenfunctions of the Bloch-Torrey operator and computed the Bloch-Torrey eigenfunctions and eigenvalues.

==> my_macros_format.tex <==
\newcommand{\HRule}{\rule{\linewidth}{0.5mm}}
\newcommand\etc{\textsl{etc}}
\newcommand\eg{\textsl{eg.}\ }
%\newcommand\etal{\textsl{et al.}}
\newcommand\Quote[1]{\lq\textsl{#1}\rq}
%%%%%\soutnew{old text we are removing}{replacement text}
%%%%%\soutnew{}{added text}
%%%%%\soutnew{remove text}{}

%%%%% for reviewers to mark the file
%\newcommand{\soutnew}[2]{\sout{#1} \uwave{#2}}

%%%%% for final latex version generation
\newcommand{\soutnew}[2]{#2}


%%%%\marginparnew{comment to reviewer}
%%%%% for reviewers to mark the file
\newcommand{\marginparnew}[1]{\marginpar{#1}}

%%%%% for final latex version generation
%\newcommand{\marginparnew}[1]{}
